Reactive atomistic simulations of Diels-Alder-type reactions: Conformational and dynamic effects in the polar cycloaddition of 2,3-dibromobutadiene radical ions with maleic anhydride

The kinetics, dynamics and conformational specificities for the ionic Diels-Alder reaction (polar cycloaddition) of maleic anhydride with 2,3-dibromobutadiene radical ions have been studied theoretically using multisurface adiabatic reactive molecular dynamics. A competition of concerted and stepwise reaction pathways was found and both the s-cis and s-trans conformers of of the diene are reactive. The analysis of the minimum dynamic path of the reaction indicates that both, rotations and vibrations of the reactant molecules are important for driving the system towards the transition state. The rates were computed as $k = 5.1 \times 10^{-14}$ s$^{-1}$ for the s-cis and $k = 3.8 \times 10^{-14}$ s$^{-1}$ for the s-trans conformer of 2,3-dibromobutadiene at an internal temperature of 300 K. The present results are to be contrasted with the neutral variant of the title system in which only the gauche conformer of the diene was found to undergo a considerably slower, concerted and mostly synchronous reaction driven by the excitation of rotations. The results presented here inform detailed experimental studies of the dynamics of polar cycloadditions under single-collision conditions in the gas phase.

==> latexmkrc <==

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

